SNP: Structured Neuron-level Pruning to Preserve Attention Scores

Multi-head self-attention (MSA) is a key component of Vision Transformers (ViTs), which have achieved great success in various vision tasks. However, their high computational cost and memory footprint hinder their deployment on resource-constrained devices. Conventional pruning approaches can only compress and accelerate the MSA module using head pruning, although the head is not an atomic unit. To address this issue, we propose a novel graph-aware neuron-level pruning method, Structured Neuron-level Pruning (SNP). SNP prunes neurons with less informative attention scores and eliminates redundancy among heads. Specifically, it prunes graphically connected query and key layers having the least informative attention scores while preserving the overall attention scores. Value layers, which can be pruned independently, are pruned to eliminate inter-head redundancy. Our proposed method effectively compresses and accelerates Transformer-based models for both edge devices and server processors. For instance, the DeiT-Small with SNP runs 3.1$\times$ faster than the original model and achieves performance that is 21.94\% faster and 1.12\% higher than the DeiT-Tiny. Additionally, SNP combine successfully with conventional head or block pruning approaches. SNP with head pruning could compress the DeiT-Base by 80\% of the parameters and computational costs and achieve 3.85$\times$ faster inference speed on RTX3090 and 4.93$\times$ on Jetson Nano.

==> table/testbeds.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|cccccc}
% \hline \hline
%                                & Device Name        & Specifications                    & Format        & Batch size & \#~Warm up       & \#~Runs                   \\ \hline
%                                & Raspberry Pi 4B    & CPU~(ARM Cortex-A72)              & Onnx          & 1          &                  &                           \\
% \multirow{-2}{*}{Edge}         & Jetson Nano        & GPU   (NVIDIA Tegra X1+)          & TensorRT      & 1          &                  &                           \\ \hline
%                                & Xeon Silver        & CPU   (Intel Xeon Silver 4214R)   & PyTorch       & 1          & 200              & 1000                      \\
% \multirow{-2}{*}{Server-based} & GeForce RTX 3090   & GPU   (NVIDIA GeForce RTX3090)    & PyTorch       & 64         & 200              & 1000                      \\ \hline \hline
% \end{tabular}}
% \label{table:testbeds}
% \end{table}

% \begin{table}[]
% \caption{\textbf{Test environments to benchmark latency.} One on a CPU and one on a GPU for both edge devices and server processors. Conventional PyTorch model is utilized for profiling on the server processor. On the Raspberry Pi 4B and Jetson Nano, profiling is performed using the ONNX and TensorRT formats, respectively.}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|c|ccccc}
% \hline \hline
%                                 & Type & Device Name               & Format (extension)        & Batch size \\ \hline
%                                 & CPU  & Raspberry Pi 4B           & Onnx (.onnx)          & 1          \\
% \multirow{-2}{*}{Edge}          & GPU  & Jetson Nano               & TensorRT (.trt)      & 1          \\ \hline
%                                 & CPU  & Intel Xeon Silver 4214R   & PyTorch (.pt)       & 1          \\
% \multirow{-2}{*}{Server}        & GPU  & NVIDIA GeForce RTX3090    & PyTorch (.pt)       & 64         \\ \hline \hline
% \end{tabular}}
% \label{table:testbeds}
% \end{table}

